An Elementary Proof of the Dvoretzky--Kiefer--Wolfowitz--Massart Inequality

The Dvoretzky--Kiefer--Wolfowitz--Massart inequality gives an upper bound on the probability that the empirical distribution function of a finite sequence of independent random variables deviates from its theoretical value. It is widely used in statistics in tests and in the production of confidence intervals. The original proof by Massart, later reformulated by Dudley, is very long and technical. Recently, Reeve slightly extends Dvoretzky--Kiefer--Wolfowitz--Massart inequality and presents an alternative, much shorter proof, that uses a continuous time martingale. We present a simpler and less technical proof of the original Dvoretzky--Kiefer--Wolfowitz--Massart inequality, based on a discrete-time martingale and Sion's minimax theorem.

==> lebStuff_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% This is Leb's usual stuff  %%%%%%%%%%%%%
%%%%%%%%  version 2, March 2026     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Maths packages
\usepackage{amsmath,amssymb,amsfonts, amsthm}
\usepackage{amscd}
\usepackage{bbm,bm} 
\usepackage{cases}
\usepackage[mathscr]{euscript}

\usepackage{comment}

\usepackage{stmaryrd}

% Packages for References and Links
\usepackage{breakcites}
\usepackage{natbib}
% hypertexnames: see the supplementary material and  https://bit.ly/2UwcJfo and https://bit.ly/2RLQVuk
\RequirePackage[colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref}


% Packages for Formatting, Layout and Diagrams
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{array}
\usepackage[small]{caption}
\usepackage{epic,eepic, epsfig, psfrag}
\usepackage{enumerate}
\usepackage{fullpage}
\usepackage{graphicx}
\usepackage[sf,bf,SF,footnotesize]{subfigure}
\usepackage{setspace}
\usepackage{tikz}
\usepackage{xcolor}

% Packages for macros
\usepackage{etoolbox}

% ----- Layout parameters -----

% Page Layout
\setlength{\textheight}{23.4cm}
\setlength{\topmargin}{-0.15in}
\setlength{\footskip}{36pt}

% ----- Layout commands -----

% Colors 
\newcommand{\teal}[1]{{\color{teal}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\orange}[1]{{\color{orange}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\purple}[1]{{\color{purple}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}

\newcommand{\purplesout}[1]{{\color{purple} \sout{#1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{conj}[theorem]{Conjecture}
 

\newenvironment{preuve}
{\begin{quote}
\par\vspace{.5\baselineskip}\noindent\footnotesize\imp{Proof.}}
{\end{quote}\nobreak\hfill$\Box$\par\vspace{.5\baselineskip}}

\newenvironment{petit}
{\par\vspace{.5\baselineskip}\noindent\footnotesize}
{\nobreak\par\vspace{.5\baselineskip}}


\newenvironment{petiteNote}
{\begin{petit} \begin{quote} \imp{Note. }}
 {\end{quote}\end{petit}}

   
 


%\newcommand{\mas}[1]{\section[#1]{\sc #1}}
%\newcommand{\mass}[1]{\subsection[#1]{\sc #1}}
%\newcommand{\masss}[1]{\subsubsection[#1]{\sc #1}}
%\newcommand{\monp}[1]{\paragraph{\sc #1}}

%%% for including pseudo code in text
\newcommand{\bp}{ % begin program
  \small \ttfamily
 \begin{tabbing}
 aaa\=aaa\=aaa\=aaa\=aaaaaaaa \= aaaaaaaaaa\= \kill
 }
\newcommand{\ep}{\end{tabbing}\normalfont\normalsize }% end program

%\newcommand{\pro}[1]{\ttfamily\small#1\normalfont\normalsize}
\newcommand{\pro}[1]{{\ttfamily\small#1}}

\newcommand{\aref}[1]{Algorithm~\ref{#1}}
\newcommand{\fref}[1]{Figure~\ref{#1}}
\newcommand{\sref}[1]{Section~\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\coref}[1]{Corollary~\ref{#1}}
\newcommand{\eref}[1]{(\ref{#1})}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\dref}[1]{Definition~\ref{#1}}
\newcommand{\lref}[1]{Lemma~\ref{#1}}
\newcommand{\thref}[1]{Theorem~\ref{#1}}
\newcommand{\pref}[1]{Proposition~\ref{#1}}
\newcommand{\pgref}[1]{Page~\pageref{#1}}
\newcommand{\qref}[1]{Question~\ref{#1}}
\newcommand{\exref}[1]{Example~\ref{#1}}
\newcommand{\exoref}[1]{Exercise~\ref{#1}}
\newcommand{\hyporef}[1]{Hypothesis~\ref{#1}}

\newcommand{\paref}[1]{Algorithm~\ref{#1} on page~\pageref{#1}}
\newcommand{\pfref}[1]{Figure~\ref{#1} on page~\pageref{#1}}
\newcommand{\psref}[1]{Section~\ref{#1} on page~\pageref{#1}}
\newcommand{\pcref}[1]{Chapter~\ref{#1} on page~\pageref{#1}}
\newcommand{\pcoref}[1]{Corollary~\ref{#1} on page~\pageref{#1}}
\newcommand{\peref}[1]{Equation~(\ref{#1}) on page~\pageref{#1}}
\newcommand{\ptref}[1]{Table~\ref{#1} on page~\pageref{#1}}
\newcommand{\pdref}[1]{Definition~\ref{#1} on page~\pageref{#1}}
\newcommand{\plref}[1]{Lemma~\ref{#1} on page~\pageref{#1}}
\newcommand{\pthref}[1]{Theorem~\ref{#1} on page~\pageref{#1}}
\newcommand{\ppref}[1]{Proposition~\ref{#1} on page~\pageref{#1}}
\newcommand{\pqref}[1]{Question~\ref{#1} on page~\pageref{#1}}
\newcommand{\pexref}[1]{Example~\ref{#1} on page~\pageref{#1}}
\newcommand{\pexoref}[1]{Exercise~\ref{#1} on page~\pageref{#1}}

\newcommand{\maketline}{\noindent \rule{16.5cm}{0.02in} \newline }
\newcommand{\makeline}{\noindent \rule{16.5cm}{0.04in}}

%\newtheorem{st}{Student Tutorial}[section]
%\newtheorem{exo}{Exercise}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{conj}{Conjecture}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{fact}{Fact}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{ex}{Example}[section]


\newcommand{\dis}{\displaystyle}
\newcommand{\ie}{{\em i.e., }}
\newcommand{\eg}{{\em e.g., }}
\newcommand{\cqfd}{\hfill $\diamond$}
%\newcommand{\qed}{\hfill{$\diamond$}}
\newcommand{\la}{\lambda}
\newcommand{\calA}{\mathcal A}
\newcommand{\calB}{\mathcal B}
\newcommand{\calC}{\mathcal C}
\newcommand{\calD}{\mathcal D}
\newcommand{\calE}{\mathcal E}
\newcommand{\calF}{\mathcal F}
\newcommand{\calG}{\mathcal G}
\newcommand{\calH}{\mathcal H}
\newcommand{\calI}{\mathcal I}
\newcommand{\calJ}{\mathcal J}
\newcommand{\calK}{\mathcal K}
\newcommand{\calL}{\mathcal L}
\newcommand{\calM}{\mathcal M}
\newcommand{\calN}{\mathcal N}
\newcommand{\calQ}{\mathcal Q}
\newcommand{\calP}{\mathcal P}
\newcommand{\calR}{\mathcal R}
\newcommand{\calS}{\mathcal S}
\newcommand{\calT}{\mathcal T}
\newcommand{\calU}{\mathcal U}
\newcommand{\calV}{\mathcal V}
\newcommand{\calX}{\mathcal X}
\newcommand{\call}{\mathcal l}
\newcommand{\calZ}{\mathcal Z}

\newcommand{\lp}{\left(}
\newcommand{\lb}{\left[}
\newcommand{\lc}{\left\{}
\newcommand{\ld}{\left.}
\newcommand{\rp}{\right)}
\newcommand{\rb}{\right]}
\newcommand{\rc}{\right\}}
\newcommand{\rd}{\right.}
\newcommand{\ib}[1]{\left \llbracket #1 \right\rrbracket}

\newcommand{\eps}{\epsilon}
\newcommand{\esp}[1]{\E\left(#1\right)}
\newcommand{\espc}[2]{\E\left(\left.#1 \right| #2\right)}

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\card}{\mbox{card}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


\newcommand{\midwor}[1]{\;\textnormal{ #1 }\;} % text in math mode

\newcommand{\nin}{\not\in} %% negation of \in
%\newcommand{\nin}{\in\!\!\!\!/} %% negation of \in
%\newcommand{\nin}{\in\!\!\/} %% negation of \in
% comb(n,p) = number of combinations of p among n
\newcommand{\comb}[2]{
 \left(
 \begin{array}{c}
    #1 \\
    #2
  \end{array}
  \right)
  }
%%% indicator functions
\newcommand{\ind}[1]{\mathbf{1}_{\{#1\}}}


 %%% norm
 \newcommand{\norm}[1]{\left\|#1\right\|}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\ben{\[}
\def\een{\]}
\newcommand{\bea}{\begin{align}}
\newcommand{\eea}{\end{align}}
\def\bean{\begin{align*}}
\def\eean{\end{align*}}
\def\bearn{\begin{eqnarray*}}
\def\eearn{\end{eqnarray*}}
\def\bear{\begin{eqnarray}}
\def\eear{\end{eqnarray}}
\def\barr{\begin{array}}
\def\earr{\end{array}}
\def\bel{\be \barr{l}}% equation array adjusted left, numbered
\def\eel{\earr\ee}
\def\beln{\ben \barr{l}}% equation array adjusted left, no number
\def\eeln{\earr\een}

\def\bfig{\begin{figure}}
\def\efig{\end{figure}}
% matrix with column formats in argument
% for example \bmat{cccc}
\def\bmat{\left(\begin{array}}
\def\emat{\end{array}\right)}

\newcommand{\erfc}{\mathrm{erfc}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\limit}[2]{\lim_{#1 \rightarrow #2}}
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}} % by definition


\newcommand{\pd}{day$^{-1}$}% per day
\newcommand{\dert}[1]{\frac{d#1}{dt}} % derivative wr t
\newcommand{\pdert}[1]{\frac{\partial#1}{\partial t}} % partial derivative wr t
\newcommand{\pder}[2]{\frac{\partial#1}{\partial#2}} % partial derivative wr 2nd arg
\newcommand{\rear}[1]{\stackrel{#1}{\rightarrow}} % reaction arrow
\newcommand{\drear}[2]{\begin{array}{c}#1\\ \rightleftarrows\\#2\end{array}} % double reaction arrow
\newcommand{\df}[1]{\textbf{#1}} % deterministic function
\newcommand{\rf}[1]{\textsf{\textbf{#1}}} % random quantity
\newcommand{\pbd}[1]{\parbox[t]{14cm}{#1}} % parbox approx 10 cm wide
%\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}} % equality as a definition

\newcommand{\vone}{\vec{1}}
\newcommand{\vzero}{\vec{0}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vmu}{\vec{\mu}}
\newcommand{\vomega}{\vec{\omega}}
\newcommand{\vtheta}{\vec{\theta}}
\newcommand{\vtau}{\vec{\tau}}
\newcommand{\va}{\vec{a}}
\newcommand{\vb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\ve}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vm}{\vec{m}}
\newcommand{\vn}{\vec{n}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vK}{\vec{K}}
\newcommand{\vX}{\vec{X}}
\newcommand{\vY}{\vec{Y}}
\newcommand{\vZ}{\vec{Z}}
\newcommand{\vV}{\vec{V}}
\newcommand{\vepsilon}{\vec{\epsilon}}
\newcommand{\vphi}{\vec{\varphi}}

\newcommand{\mif}{\mathrm{\; if \; }}
\newcommand{\mthen} {\mathrm{\;  then \;  }}
\newcommand{\melse} {\mathrm{\;  else \;  }}
\newcommand{\mand} {\mathrm{\;  and \; }}
\newcommand{\mor} {\mathrm{\;  or \; }}
\newcommand{\mst} {\mathrm{\;  such \;  that \; }}
\newcommand{\mfa} {\mathrm{\;  for \;  all \; }}
\newcommand{\mfor} {\mathrm{\;  for \;  }}
\newcommand{\mf} {\mathrm{\;  for \; }}
\newcommand{\mfs} {\mathrm{\;  for \; some \; }}
\newcommand{\moth} {\mathrm{\;  otherwise \; }}
\newcommand{\mwith} {\mathrm{\;  with \; }}

\def\I{I\!d}
\def\Reals{\mathbb{R}}
\def\Rats{\mathbb{Q}}
\def\Ints{\mathbb{Z}}
\def\Comps{\ensuremath{\mathbb{C}}}
\def\GF{\ensuremath{\mathbb{F}}}
\newcommand{\ints}[1]{{\Ints/#1\Ints}}
\def\Nats{\mathbb{N}}
\def\E{\mathbb{E}}
\def\P{\mathbb{P}}
\def\T{\mathbb{T}}
\def\Abb{\mathbb{A}}
\def\mpc{\otimes}
\def\mpd{\oslash}
\def\Mpc{\overline{\otimes}}
\def\Mpd{\overline{\oslash}}

\newcommand{\cro}[1]{\langle#1\rangle}   % bracket for integrals etc
\newcommand{\bra}[1]{\lb#1\rb}   % modulo class
% ajoute LEB 2001.01.11 to compile netcal book
\def\mod{\bmod}
\def\hdots{\cdots}

 
\newcommand{\bracket}[1]{ \left\{\begin{array}{l} #1 \end{array} \right.}
\newcommand{\gap}{\,\,\,}

 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%  End of Leb's usual stuff  %%%%%%%%%%%%%
%%%%%%%%                            %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

